Lithography Hotspot Detection via Heterogeneous Federated Learning with Local Adaptation

As technology scaling is approaching the physical limit, lithography hotspot detection has become an essential task in design for manufacturability. While the deployment of pattern matching or machine learning in hotspot detection can help save significant simulation time, such methods typically demand for non-trivial quality data to build the model, which most design houses are short of. Moreover, the design houses are also unwilling to directly share such data with the other houses to build a unified model, which can be ineffective for the design house with unique design patterns due to data insufficiency. On the other hand, with data homogeneity in each design house, the locally trained models can be easily over-fitted, losing generalization ability and robustness. In this paper, we propose a heterogeneous federated learning framework for lithography hotspot detection that can address the aforementioned issues. On one hand, the framework can build a more robust centralized global sub-model through heterogeneous knowledge sharing while keeping local data private. On the other hand, the global sub-model can be combined with a local sub-model to better adapt to local data heterogeneity. The experimental results show that the proposed framework can overcome the challenge of non-independent and identically distributed (non-IID) data and heterogeneous communication to achieve very high performance in comparison to other state-of-the-art methods while guaranteeing a good convergence rate in various scenarios.

==> _tex/3_problem.tex <==
%=======================================%
%                 Problem.              %
%=======================================%

\section{Problem Formulation} % or Motivation

\begin{table}[tb!]
    \centering
    \caption{Nomenclature.}
    \label{tab:nomenclature}
    %\resizebox{0.85\linewidth}{!}
    {
        \begin{tabular}{c|l}
            \toprule
            Symbol & Definition \\ \midrule
            $w$ & Weights of a DNN model. \\
            $w_{g}$ & Global weights of  model. \\
            $w_{l}^{k}$ & Local weights of the $k$-th client model. \\
            $N$ & Total number of clients. \\
            $n_{k}$ & The sample size of the $k$-th client.\\ \bottomrule
        \end{tabular}
    }
\end{table}

% Nomenclature
We use the nomenclature shown in Table~\ref{tab:nomenclature} to formulate our problem.

The performance of a hotspot detector can be evaluated by the true positive rate (TPR), which is also referred to as recall or sensitivity, the false positive rate (FPR), and the overall accuracy.

% \begin{namedthm*}{Definition 1} [{\bf true positive rate}]
% The ratio between the number of correctly identified layout hotspots and the total number of hotspots.
% \end{namedthm*}

% \begin{namedthm*}{Definition 2} [{\bf false positive rate}]
% The ratio between the number of wrongly identified layout hotspots (false alarms) and the total number of non-hotspot clips.
% \end{namedthm*}

\begin{namedthm*}{Definition 1} [{\bf accuracy}]
The ratio between the number of correctly classified clips and the total number of clips.
\end{namedthm*}

With the evaluation metrics above, our problem is formulated as follows.

% Give other definitions

% Give problem formulation using our definitions

\begin{namedthm*}{Problem 1} [{\bf Hotspot Detection}]
The inputs of every client are circuit layout data containing hotspot, non-hotspot layout patterns and their labels. Clients frequently generate and collect circuit layout data in a highly non-identically distributed manner. The objective of distributed hotspot detection is training a model under the non-IID settings to learn optimal features and classify all the clips so that the model can maximize the accuracy and minimize the false  positive  rate.
\end{namedthm*}



